Speech2Face: Learning the Face Behind a Voice

How much can we infer about a person's looks from the way they speak? In this paper, we study the task of reconstructing a facial image of a person from a short audio recording of that person speaking. We design and train a deep neural network to perform this task using millions of natural Internet/YouTube videos of people speaking. During training, our model learns voice-face correlations that allow it to produce images that capture various physical attributes of the speakers such as age, gender and ethnicity. This is done in a self-supervised manner, by utilizing the natural co-occurrence of faces and speech in Internet videos, without the need to model attributes explicitly. We evaluate and numerically quantify how--and in what manner--our Speech2Face reconstructions, obtained directly from audio, resemble the true face images of the speakers.

==> sec1_introduction_backup.tex <==
\section{Introduction}
% Intro.
\noindent
When we listen to a person speaking without seeing his/her face, on the phone, or on the radio, we often build a mental model for the way the person looks~\cite{kamachi2003putting,smith2016matching}. There is a strong connection between speech and appearance, part of which is a direct result of the mechanics of speech production: age, gender (which affects the pitch of our voice), the shape of the mouth, facial bone structure, thin or full lips---all can affect the sound we generate. \tali{Following on Tae-Hyun comment, we need a citation here.} In addition, other voice-appearance correlations stem from the \emph{way} in which we talk: language, accent, speed, pronunciations---such properties of speech are often shared among nationalities and cultures, which can in turn translate to common physical features~\cite{denes1993speech}. 
%Both auditory and visual information are known to be important for the perception of speech. 


% This work.
% Our goal in this work is to study to what extent we can infer how a person looks---specifically a person's face---from the way they talk.
Our goal in this work is to study to what extent we can infer how a person looks from the way they talk. Specifically, from a short input audio segment of a person speaking, our method directly reconstructs an image of the person's face in a canonical form (i.e., frontal-facing, neutral faces). Fig.~\ref{fig:teaser} shows sample results of our method.  Note that our goal is not to predict a recognizable image of the exact face (nor do we believe it is possible), but rather capture dominant facial traits of the person that are correlated with the input speech.
%This problem and capability, we argue, are not just interesting to explore academically, but can also support useful applications as we will discuss shorty.
%And we'd only expect the model to capture typical correlations between speech and appearance. For example, predicting a person's hairstyle is not expected, as it is likely less correlated with speech in videos.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/teaser2.pdf}
    \caption{\emph{Top:} We consider the task of reconstructing an image of a person's face from a short input audio segment of speech. \emph{Bottom:} several results of our method are shown. The true faces are shown just for reference; our model takes only an audio waveform as input. Note that our goal is not to reconstruct an accurate image of the person, but rather to recover characteristic physical features that are correlated with the input speech. All our results  including the input audio, are available in the supplementary material (SM).}
    \label{fig:teaser}\afterfig
\end{figure}

\begin{figure*}[t!]
\vspace{-.2in}
\centering
\includegraphics[width=1\textwidth]{figures/pipeline2.pdf}
\caption{{\bf Speech2Face model and training pipeline.} The input to our network is a complex spectrogram computed from the short audio of a person speaking. The output is a 4096-D face embedding that is then decoded into a canonical image of the face using a pre-trained face decoder network~\protect\cite{cole2017synthesizing}. The part we train is marked by the orange-tinted box. We train the network to regress to the true face embedding computed by feeding an image of the person (representative frame from the video) into a face recognition network~\cite{Parkhi15} and extracting the feature from its penultimate layer. Our model is trained on millions of speech--face embedding pairs from the AVSpeech dataset~\cite{ephrat2018looking}.}
\label{fig:pipleine}\afterfig
\end{figure*}
% Method.

We design a deep network model that takes the complex
spectrogram of a short speech segment as input and predicts
a feature vector representing the face. More specifically, the
predicted face feature represents a 4096-D face embedding that is extracted from the penultimate layer (i.e., one layer prior to the classification layer) of a pre-trained face recognition network~\cite{Parkhi15}. We decode the predicted face feature into a canonical image of the person's face using a separately-trained reconstruction model~\cite{cole2017synthesizing}. To train our model, we use the AVSpeech dataset~\cite{ephrat2018looking}, comprised of millions of video segments from YouTube with more than 100,000 different people speaking. Our method is trained in a self-supervised manner, i.e., it simply uses the natural co-occurrence of speech and faces in videos, not requiring additional information, e.g., human annotations. %All that is required for training are the speech waveforms and video frames.

% Compared to predicting attributes.
We are certainly not the first to attempt to infer information about people from their voices. For example, predicting age and gender from speech has been widely explored~\cite{zazo2018age,hansen2015speaker,feld2010automatic,bahari2011speaker,wen2018disjoint}.
Indeed, our goal of producing a face image representing an input voice could be achieved via an alternative approach by first predicting some attributes about the person of the voice (e.g., their age, gender, etc.; see Zazo et al.~\cite{zazo2018age} for instance), and then either fetching an image from a database that best fits the predicted set of attributes, or using the attributes to generate an image~\cite{yan2016attribute2image}.
% Indeed, if our goal is to produce a face image matching an input voice, an alternative approach to ours may be to first predict some attributes about the person (their age, gender, etc., e.g.,~\cite{zazo2018age}), then fetch an image from a database that best fit the predicted set of attributes, or rather use the attributes to generate an image~\cite{yan2016attribute2image}.
% \miki{TH, you mentioned~\cite{ohsugi2018comparative}, how is it related here? it seems to do the other direction}
% \oh{Right, it's the other way around. If you feel this is not suitable, we can drop. The work was a response for what you asked, ``retrieval style face2speech association'' as an alternative approach.  \cite{ohsugi2018comparative} constructs a match from a face to a voice style. While they emphasized face $\rightarrow$voice, their approach actually does not have a limitation to be voice $\rightarrow$face as long as a mapping database is maintained, I put this reference in this consideration, but it is indeed too indirect. Other than this, we may use \cite{kim2018on}.}
However, there has been little work on predicting visual appearance, e.g., a face image, directly from speech. We argue that such an approach is important and relevant to study for the following two reasons.

%\begin{enumerate}

%\item 
First, predicting attributes from an input signal requires the existence of robust and accurate  classifiers and often requires ground truth labels for supervision. For example, predicting age, gender, or ethnicity, from speech requires building classifiers specifically trained to capture those properties. In contrast, voices and corresponding images of speakers are naturally coupled and widely available in videos on the Web. This allows us to train a model that translates speech features to visual features directly and at scale. The reconstructed face images can be used as a proxy to convey the visual properties of the person, without requiring explicitly trained classifiers for every attribute we want to capture.


%\item 
Second, in addition to asking to what level of detail we can recover how a person looks from their voice---an interesting scientific question worthy of studying on its own---we believe the face images we recover from speech may also support useful applications. These can include attaching a representative face to a person in phone/video calls where the person may not wish to share their picture or video feed. Other uses may include forensic applications, helping to establish visual profiles of people from phone recordings. In such cases, our technique can reconstruct face images directly from the input speech in a single shot, without the need to first predict a discrete set of attributes, then translate them to a face image.
%\end{enumerate}

To our knowledge, our paper is the first to explore learning to reconstruct face images directly from speech. We test our model on various speakers and present qualitative results.
% To our knowledge, our paper is the first to explore self-supervised learning for reconstructing face images directly from speech. We test our model on various speakers and present qualitative results and well as an \oh{let me remove `thorough'} ablation study of our model. \changil{We do not have an ablation study for now.}
We also show numerically that our reconstructed face images agree well with the true images of the speakers (unknown to the method, only used for evaluation) in terms of age, gender, and ethnicity. Beyond these dominant attributes, we also notice in some cases that our reconstructions capture finer facial properties (e.g., the width of the face). %We believe that genera

%---attributes for which robust, commercial classifiers exist. \changil{This last part of the sentence seems contradicting to the point 1, dictating the age/gender/etc.\ classifiers are hindering the alternative approach. I commented it out for now.}
%In addition to those dominant attribute We also observe the are model is able to capture finer grained properties such as elongated vs. round heads and BMI.


%We leave a more thorough evaluation of the practical applications for future work, by us and by others.


%$scientifically, we would like to see if predicting images may facilitate inferring properties that are not easily captured by a discrete set of classifiers.
%And we can produce those images directly in a single shot rather than first predicting attributes and then translating those to a representative face.





